IKEA-Manual: Seeing Shape Assembly Step by Step

Human-designed visual manuals are crucial components in shape assembly activities. They provide step-by-step guidance on how we should move and connect different parts in a convenient and physically-realizable way. While there has been an ongoing effort in building agents that perform assembly tasks, the information in human-design manuals has been largely overlooked. We identify that this is due to 1) a lack of realistic 3D assembly objects that have paired manuals and 2) the difficulty of extracting structured information from purely image-based manuals. Motivated by this observation, we present IKEA-Manual, a dataset consisting of 102 IKEA objects paired with assembly manuals. We provide fine-grained annotations on the IKEA objects and assembly manuals, including decomposed assembly parts, assembly plans, manual segmentation, and 2D-3D correspondence between 3D parts and visual manuals. We illustrate the broad application of our dataset on four tasks related to shape assembly: assembly plan generation, part segmentation, pose estimation, and 3D part assembly.

==> fig_texts/geocluster.tex <==
\begin{algorithm}
\caption{GeoCluster}\label{alg:geocluster}
\begin{algorithmic}
\Require Parts $\{P_1, \cdots, P_n\}$
\Ensure An assembly tree $T$
\Procedure{Group}{$I$}
\State partition $I$ into clusters $\{C_1, \cdots, C_m\}$ based on DGCNN~\cite{wang2019dynamic} features of $\{P_i\}_{i\in I}$%
\If{clustering fails}
\State\Return a node with children $I$
\EndIf
\State choose cluster $C^\ast$ with minimum in-cluster feature variance
\State\Return a node with children $C^\ast \bigcup\{\Call{Group}{I \setminus C^\ast}\}$
\EndProcedure
\State\Return \Call{Group}{$\{1, \cdots, n\}$}
\end{algorithmic}
\end{algorithm}


==> fig_texts/web.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figs/web.png}
    \caption{Our web-based interface for manual-related annotation. It provides functionality to annotate the assembly plan, segmentation and 2D-3D correspondences in a unified environment.}
    \label{fig:web}
\end{figure}
